A Bayesian Evaluation Framework for Subjectively Annotated Visual Recognition Tasks

An interesting development in automatic visual recognition has been the emergence of tasks where it is not possible to assign objective labels to images, yet still feasible to collect annotations that reflect human judgements about them. Machine learning-based predictors for these tasks rely on supervised training that models the behavior of the annotators, i.e., what would the average person's judgement be for an image? A key open question for this type of work, especially for applications where inconsistency with human behavior can lead to ethical lapses, is how to evaluate the epistemic uncertainty of trained predictors, i.e., the uncertainty that comes from the predictor's model. We propose a Bayesian framework for evaluating black box predictors in this regime, agnostic to the predictor's internal structure. The framework specifies how to estimate the epistemic uncertainty that comes from the predictor with respect to human labels by approximating a conditional distribution and producing a credible interval for the predictions and their measures of performance. The framework is successfully applied to four image classification tasks that use subjective human judgements: facial beauty assessment, social attribute assignment, apparent age estimation, and ambiguous scene labeling.

==> graphics/exp3/supp_mat/auc_table.tex <==
\begin{table*}[h]
\begin{center}
\begin{tabular}{|l|llll|llll|llll|llll|}
    \hline
    & \multicolumn{4}{c|}{LabelMe} & \multicolumn{4}{c|}{SCUT-FB5500} & \multicolumn{4}{c|}{APPA-REAL} & \multicolumn{4}{c|}{TestMyBrain: Trust} \\
    & \multicolumn{4}{c|}{Predictor Epochs} & \multicolumn{4}{c|}{Predictor Epochs} & \multicolumn{4}{c|}{Predictor Epochs} & \multicolumn{4}{c|}{Predictor Epochs} \\
    & 0 & 7 & 14 & 100
        & 0 & 3 & 7 & 60
        & 0 & 1 & 2 & 100
        & 0 & 1 & 2 & 100 \\
    \hline
    \textit{Train}: & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} \\
    AUC
        & .49 & .88 & .99 & .99
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    Lower
        & .49 & .88 & .99 & .99
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    Upper 
        & .49 & .88 & .99 & .99
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    \hline
    \textit{Test}: & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} & \multicolumn{4}{c|}{} \\
    AUC
        & .49 & .87 & .89 & .89
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    Lower
        & .49 & .88 & .99 & .99
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    Upper
        & .49 & .88 & .99 & .99
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60
        & 0 & 3 & 7 & 60 \\
    \hline
\end{tabular}
\end{center}
%\vspace{-6mm}
\caption{
    The values of the original AUC and the lower and upper bounds of the BNN's highest density credible interval as visualized in Supp. Mat. Fig \ref{fig:exp3_auc}.
}
\label{tab:auc}
\end{table*}

==> writing/6_broader_impact.tex <==
\section{Broader Impact}

This research was motivated by the social concerns surrounding 
predictors for ground truth-free visual recognition tasks --- many of which have questionable uses. For instance, consider an application of personality attribute prediction for job candidate assessment that takes into account the attribute of enthusiasm. This is a real example of the general class of technology we consider in this paper, which is being deployed without the vetting necessary to ensure that it is operating in a socially acceptable manner~\cite{burke_2019}. Such a technology may unfairly rate as unenthusiastic older workers, people with disabilities, and people of color if the predictors were only trained on noisy data that lead to uncertain predictions for these demographics. Compared to assessments made by fair human interviewers who are attuned to differences across demographics, this outcome would be completely unacceptable. In order to avoid a problem like this, it would be important to know if predictors used in this application are behaving erratically.
%This information can be used to formulate a coherent and effective policy to regulate the use of the technology so that it only operates in a manner deemed correct by all stakeholders. 
Below we take a brief look at the potential positive and negative outcomes of our work in this context.

%\textbf{A)
Who may benefit from this research? Both researchers and practitioners working on ground truth-free visual recognition tasks will benefit from this work, as it provides a fruitful path forward for improving the operational performance of trained predictors in an otherwise difficult setting for evaluation. Moreover, policy and standards experts can also make use of this research in order to falsify claims of human-like performance. On the opposite end of the spectrum, it will be possible to find predictors that may be of concern due to their remarkably good performance on socially sensitive tasks, where they could be used to fool humans (\textit{e.g.}, social engineering bots). Finally, this research will be particularly attractive to the affective computing community, where social attribute predictors can have a large impact in work on autism and other developmental disorders. 

%\textbf{B)
Who may be put at disadvantage from this research? As this paper presents work on evaluation specifically aimed at addressing problems in work on ground truth-free problems, it is not immediately clear if any populations are put at a disadvantage because of it. One potential area of concern is that a failure in proper implementation of the framework causes an unanticipated consequence along these lines. This is addressed in the next point.

%\textbf{C)
What are the consequences of failure of the system? Failure modes in the proposed evaluation framework may misrepresent the performance of a predictor being tested. This could portray it as operating better or worse than it does on average in practice, with respect to human annotator behavior on the same task. However, given that this is a framework, where various pieces can be configured in different ways, a suite of tests can be deployed to mitigate this concern. While failure may be the result of one configuration of the framework, the examination of the output for multiple runs with different configurations may provide a clearer picture of a predictor's performance.

%\textbf{D)
Whether the task/method leverages biases in the data?
This is an interesting question in the context of ground truth-free predictors. For the tasks these predictors are trained to perform, the objective is often to match human performance, biases included. Thus if we are trying to compare predictors to human annotator behavior, an evaluation procedure with a learning component, such as the BNN configuration of our framework, must necessarily capture these biases as well. However, given that this is not an unintended consequence, it isn't necessarily a problem --- especially if a population of fair human annotators is being used for comparison. How the predictors are used is a larger concern. Thus any biases that exist within the human annotators should be identified and disclosed before deployment of predictors that make use of that data.
